Unit Region Encoding: A Unified and Compact Geometry-aware Representation for Floorplan Applications

We present the Unit Region Encoding of floorplans, which is a unified and compact geometry-aware encoding representation for various applications, ranging from interior space planning, floorplan metric learning to floorplan generation tasks. The floorplans are represented as the latent encodings on a set of boundary-adaptive unit region partition based on the clustering of the proposed geometry-aware density map. The latent encodings are extracted by a trained network (URE-Net) from the input dense density map and other available semantic maps. Compared to the over-segmented rasterized images and the room-level graph structures, our representation can be flexibly adapted to different applications with the sliced unit regions while achieving higher accuracy performance and better visual quality. We conduct a variety of experiments and compare to the state-of-the-art methods on the aforementioned applications to validate the superiority of our representation, as well as extensive ablation studies to demonstrate the effect of our slicing choices.

==> Sections/11_intro.tex <==
\section{Introduction}
Floorplan plays an essential role in architecture designs and analysis. Over the past decades, there has been a dramatic increase in the related research area, such as floorplan generation, scene synthesis, and scene understanding(-----------reference-------------). These works take floorplans as input and generate both realistic and diverse 2D or 3D content. The floorplan is a polygon shape expressed as a vector of vertices. The bounded inner space of the polygon would be the semantic field for different tasks, e.g., segmentation, classification, and generation. This indicates that all the information of the semantic field is derived from the geometry shape of floorplans. However, previous works simply take the semantic field, which is a binary mask, as inputs without explicit geometry information. Recent advances in structural similarity(-----------reference-------------) emphasize structures of the floorplan and represent as a graph but with hand-craft geometrical features. Another line of research related to geometric shapes represents the contour directly as a vector of vertices or scalable vector graphics(SVG) while not concerned with the inner semantic regions. 


 	Despite these efforts, there have been very few attempts to represent and utilize both geometric and semantic information. In this work, we propose a novel floorplan representation that explicitly introduces geometric information into the semantic floorplan regions; see Figure ~\ref{fig:teaser} for an overview of our framework. Specifically, we reformulate the floorplans as variants derived from the base floorplan, a regular quadrilateral. The variants are performed by the "squeeze" operation. Each operation would alter the geometric shape and differentiate the density of the inner space. By grouping spaces with the same density(i.e., the same geometric characteristics), we generate a set of regions(called uniform regions). 


	Moreover, when we use these coarse regions to represent the 3D-FRONT and RPLAN datasets[----reference----] by assigning a label(e.g., room id or type), we observe a strong correlation (0.95 for 3D-FRONT and 0.65 for RPLAN) between the Uniform Regions and original datasets. This means the granularity on floorplan-related tasks is over-segmented by pixel level. Therefore, there will be a great potential for decreasing the solution space by utilizing the Unifor Regions. Also, the density map is a new dense geometric feature, and the experiment shows a promotion when utilized as inputs.


	As for training Uniform Regions, We utilize an encoder-decoder network to generate a dense neural field from the raster floorplan image and utilize region pooling to extract features of each uniform region mapped on the image plane. Intuitively, the network is trained in a structured architecture, where the floorplan information is not learned by pixels but by regions. This would significantly decrease the learning space and result in better performance. Besides, the region is naturally defined with vector format against the primarily used vector-raster-vector pipeline, and there wouldn't be a vectorization problem. Furthermore, in practice, each uniform region is split into many sub-uniform regions to make the representation more flexible for multiple coarser or finer applications.


  We present comprehensive experiments on the 3D-Front[-reference--] with semantic segmentation task to show that with the uniform regions, the scale of the problem gets hundreds of times decreased. The qualitative and quantitative results demonstrate significant improvements. We also explore the effect of different splitting strategies of sub-uniform regions. To indicate the representation ability towards geometric shape, we show the experiment on floorplan retrieval tasks[reference--] using the RPLAN dataset[----reference--]. We represent each room as a uniform region and utilize a symmetric function to get the global features of the whole floorplan. The features are then trained under a triplet network setting. The result shows great improvements and indicates a more global and complete geometric representation. To this end, we explore the ability of the floorplan generation based on this representation. We naturally adopt a one-stage instance segmentation pipeline to segment and classify tooms. Specifically, the uniform regions are trained to be clustered into rooms and assigned room types; To enrich the distinctiveness between uniform regions, we utilize another adversarial neural network to generate a wall mask which would be a condition of the instance segmentation neural network. We demonstrate with a variety of results, user studies have shown that the generating results are competitive to those created by humans.

==> Sections/13_method.tex <==
\section{Floorplan Reformulation}

The geometric shape of floorplans varies, and the diversity constructs the space of the floorplan. We reformulate the floorplan space as operations on the base floorplan and explore the properties of each floorplan instance. 

\subsection{Uniform Regions}
Let us consider $Set_{floor}=\{S_1, S_2\dots, S_i, \dots\}$ as the space of floorplans. As ilustated in Figure \ref{fig:teaser} top, in this space, we define: 

1) \textbf{a coordinate $C$} with two directional axis as $x\ and\ y$ which correspond to west-east and south-north in reality. The coordinate leads that the base floorplan would be a regular quadrilateral with size $W$. We denote the \textbf{base floorplan as $S_0$};


2) \textbf{an operator $f(S_i, \theta)$} named $squeeze$, the operator $squeeze$ takes a floorplan $S_i$ and parameters $\theta$ as input and generate a new floorplan, where $\theta$ denotes the $squeeze$ start point, end point, and directional squeezing depth.


Each floorplan in the space would be generated by a sequence of operations:
\begin{equation}
  S_i=\left(f^j(S_0, \theta_j)\right)^N_{j=1}.
\end{equation}
Under such a formulation, we could build a relation between the contour and inner space: For the base floorplan $S_0$, it has a uniform density which means the geometric information of the inner space is uniform everywhere. While each $squeeze$ operation would change the contour shape and squeeze part of the inner space, therefore leads a differentiation of the density in the inner space. The density of regions affected gets increased according to the parameters $\theta_j$. We can form several isolated uniform regions by clustering the regions with the same density. 

\subsection{Correlation with Tasks}
The motivation of Uniform Regions is that when human designers involve with architecture applications(e.g., interior design or floorplan generation), they generally take the geometric structure of the contour as a reference and locate the bounds of room or furniture along with the corners of the contour. The alignment between geometry and applications internally follows design aesthetics. Meanwhile, the geometry-awarded Uniform Regions form a much coarser floorplan representation than pixels and follow the geometric shape's alignment. The intrinsic indicates that the new representation could better leverage the geometric information.


We observe the evidence that a strong correlation exists in the 3D-FRONT and RPLAN datasets between the Uniform Regions and the ground truth labels. Instead of assigning a label for each pixel, we split the floorplan into Uniform Regions and assigned a label for each region using the most voted value. The coarser representation with Uniform Regions will obviously cause information loss, but the loss is not so much as shown in Table. We evaluate the mean IoU as the correlation between the data with region labels under new representation and the original pixel labels. The result shows a high IoU value, 0.95 and 0.65, for 3D-FRONT and RPLAN datasets, respectively. The reason for the IoU gap between the two tasks is that the task in  3D-FRONT has a more deterministic solution than the RPLAN, and we will state the detail of the datasets in a later paragraph. The figure shows the quantitative examples.


The high correlation indicates a great potential exists for reducing the solution space by grouping pixels into regions in an appropriate way. We utilize the Uniform Regions to split the floorplan into regions, and in practice, we uniformly split each uniform region into $m\times n$ grids, named sub-Uniform Regions considering the minimal thresh in real scale, i.e., the grid nums may be adjusted and depends on that the size of each sub-Uniform Region must greater than minimal thresh with meter unit. The global defined $m\times n$ among all Uniform Regions ensures the alignment between the adjacent sub-uniform Regions from different Uniform Regions. The finer-grained splitting enhances the flexibility of the representation and, as shown in Table, only introduces minor complexibility compared with pixel representation. [---Figure---] demonstrates the visualization of different splitting granularity. We also explore the effect of different splitting strategies of sub-Uniform Regions on performance in experiments.

\begin{table}[tp]
   \fontsize{6.5}{8}\selectfont  
   \centering  
  \caption{Statistics for different sub-Unit Regions splitting strategies. We report the IoUs with ground truth and the average region numbers under different strategies.}
  \label{tab:sub_region_split}
  \begin{tabular}{lcc|cc|cc}

    \toprule
    \multirow{3}*{Strategy} & \multirow{3}*{Grid} & \multirow{3}*{Thresh} &
    \multicolumn{2}{c|}{3D-FRONT[-REF-]} & \multicolumn{2}{c}{RPLAN[-REF-]} \\
    \cline{4-7}
     {} & {} & {} &IoU&Avg. Num & IoU$(\uparrow)$ & Avg. Num$(\downarrow)$ \\
    \midrule
    \textbf{[1]Unit Region} & 1$\times$1 & 1.0m & 95.28&8.76&65.42&14.26\\
    \textbf{[2]sub-Unit Region} & 2$\times$ 2& 1.0m& 97.83&19.33&81.40&36.52\\
    \textbf{[3]sub-Unit Region} & 4$\times$ 4& 1.0m& 99.40&34.66&90.52&71.15\\
    \textbf{[4]sub-Unit Region} & 8$\times$ 8& 1.0m& 99.1&40.41&93.47&88.72\\
    \textbf{[5]sub-Unit Region} & 4$\times$ 4& 0.5m& 99.39&66.35&91.32&133.24\\
    \textbf{[6]sub-Unit Region} & 8$\times$ 8& 0.5m& 99.98&124.89&95.99&266.53\\
    \textbf{[7]Pixel-256} & - & - & 100&24137.18    &100 &17075.31    \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Density Map}
The density of the floorplan describes the degree of tightness after squeezing. Each point in the inner space will be affected by the global $squeeze$ operation and this leads a densely expressed and globally awared geometric information. We form the information into the \textbf{Density Map}. This map provides a new dense features for embedding the geometric information into semantic map. This feature enhances the performence on multiple tasks in experiments.


In fact, the \textbf{Density Map} is a variant from Signed Distance Function(SDF)[---reference---]: if $\Omega$ is a subset of a metric space, $X$, with metric, $d$, then the SDF, $f$, is defined by
\begin{equation}
  f(x)=\left\{
    \begin{aligned}
      &d(x, \partial\Omega) & \ if x \in \Omega \ &\\
      &-d(x,\partial\Omega) & \ if x \in \Omega^c&\ \ ,
    \end{aligned}
  \right.
\end{equation}
where $\partial\Omega$ denotes the boundary of $\Omega$. For any $x \in  X$,
\begin{equation}
  d(x, \partial\Omega):=\mathop{inf}\limits_{y\in \partial\Omega}d(x, y),
\end{equation}
where $inf$ denotes the infimum. We modify the metric by sum the distances to boundary along two oposite directions and set the region outside $\Omega$ as 0:
\begin{equation}
  f(x)=\left\{
    \begin{aligned}
      &d(x, \partial\Omega, \bold v) & \ if x \in \Omega \ &\\
      &0 & \ if x \in \Omega^c&\ \ ,
    \end{aligned}
  \right.
\end{equation}
\begin{equation}
  d(x, \partial\Omega, \bold v):=\mathop{inf}\limits_{y\in \partial\Omega^{\bold v+}}d(x, y) + \mathop{inf}\limits_{y\in \partial\Omega^{\bold v-}}d(x, y) \ ,
\end{equation}
where $\bold v\in [\bold x, \bold y]$, denotes that we calculate two directions along the coordinate's axis $\bold x \ and \ \bold y$. As a result, we generate two density maps. Intuitively, each $squeeze$ operation would indeed alter the density in two directions: the squeezing direction and the perpendicular direction, as shown in Figure \ref{fig:teaser} top. Therefore, the density needs to be evaluated by two directions along the $x$ and $y$ axis in coordinate $C$. The value of this map indicates the available space along each axis. Specifically, we calculate the density for each point in the inner space by measuring the distance between the two extreme points along the two axes. [----Figure---]

\section{Network Architecture}
Our full network architecture is visualized in [---Figure--], where the segmentation network, metric learning network, and the floorplan generation network share a great portion of structures. The network has three key modules: the feature fusion module for raster floorplan mask and Density Map, the Region Pooling layer to aggregate features from global floorplan centered in each region, the adaption heads for multiple tasks.

\subsection{Local and Global Information Aggregation}
The Uniform Regions describes the global floorplan in a set of local regions, while most tasks need the sense of global floorplan information. Therefore, the features of regions should combine local and global knowledge. We achieve this by utilizing an Encoder-Decoder structure. The encoder module gradually reduces the feature maps and captures high dimensional semantic information, and the decoder module gradually recovers the spatial information from the encoding features. 

The Encoder-Decoder consumes the raster floorplan mask and density map, and generates a feature map. The features in each Uniform Regions are locally centered and merge the global information with the perceptual field of convolution. These features named \textbf{Dense Neural Field} could be partially fetched according to the pre-defined Uniform Regions to represent corresponding regions. Note that the Uniform Regions are defined in vector format, and we can easily use the rasterization procedure to build a map function between the vector-format region onto the \textbf{Dense Neural Field}. Moreover, the Encoder-Decoder module plays a feature extractor role for the floorplan and thoroughly represents the floorplan in vector format. The Encoder-Decoder can be selected from previous excellent segmentation networks, and we experiment several networks including: the Deeplab v3+ [--reference--], HR-Net[--reference--], and U-Net[--reference--].

To unify the size of features from different Uniform Regions, we utilize Region Pooling to pool each channel of the features among the region into a scalar. As a result, each region is represented as a vector $f_i\in\mathbb{R}^m $. Since some floorplans may contain sloping walls, we take the regions connected by a continuous sloping wall into one Uniform Region(see [---Figure--] for an example). The Region Pooling is modified from RoI Pooling[---reference---] and supports irregular shapes.

The newly introduced Density map feature is considered to provide extra geometric information and improve performance. A direct method is an early fusion that concatenates the maps into the input as multi-channel data. While as described in [---reference--], the values of this map indicate the available space and vary in range from zero to image's resolution. Compared with the raster mask, the information on this map is much richer and will mislead the network to ignore the raster mask. Besides, the essential information in this map is the contrasts between different densities, but not the density value.

We consider a late fusion architecture where we utilize two Encoder-Decoder independently for the raster mask and the Density Maps to generate two feature maps. The feature maps are concatenated as the Dense Neural Field. Then we use several shared MLP layers to classify into a set of categories. Decoupling the raster mask and Density Maps allows us to exploit the features in different domains and experiments show improvements.



==> Sections/14_results.tex <==
\subsection{Adaption for Tasks}
After Region Pooling, the floorplan is represented as a sequence of vectors $f=[f_0, f_1,\dots] \in \mathbb{R}^{n\times m}$ from each Uniform Regions, while for different tasks, these features should be organized to adapt different tasks.


\textbf{Semantic Segmentation.} Based on the above region-based representation, we naturally assign a label for each sub-Uniform Region and train the network to classify each region instead of pixel. We add several shared MLP layers on the pooled features for classification. The loss function os modeled as the croos-entropy, which is commonly used for segmentation.


\textbf{Metric Learning.} For tasks that need to evaluate the similarity for floorplans(e.g., floorplan retrieval), a regular pipeline is to represent the floorplan in vector space and train the vector by metric. We need an operation $g([f_0, f_1,\dots])$ to extract the global features for each floorplan. A challenge when using the region-based representation is, each floorplan is expressed by multiple region features, while the numbers of regions in different floorplans are usually different. Therefore, the operation $g(\cdot)$ must accept a variable quantity of regions. Besides, the feature sequence $f=[f_0, f_1,\dots] \in \mathbb{R}^{N\times m}$ in fact is unordered, it requires the operation $g(\cdot)$ to be robust with respect to input permutation and corruption.

We find this problem is highly related with Pointnet[---reference---], the symmetric function solution is adopted:
\begin{equation}
  g([f_0, f_1,\dots,f_i,\dots, f_N]) = f_g,
\end{equation}

where $f_i \in \mathbb{R}^m, f_g\in \mathbb{R}^m, g: \mathbb{R}^{N\times m}\to \mathbb{R}^m$. 

The symmetric function is very simply implemented by an element-wise max pooling function while very efficient. The features $f_g$ are then utilized for training the similarity in a triplet setting for floorplan retrieval.

\textbf{Floorplan Generation.} As described in [---related works----], this application is usually achieved by a GAN-based semantic segmentation or two-stage object instance segmentation pipelines. Since the number of elements significantly decreases when represented by regions compared with pixels, it becomes possible to formulate this problem as single-stage instance segmentation. 

Our Encoder-Decoder architecture first extracts descriptive features for each region in the floorplan. We enforce the single-stage instance segmentation that the regions belonging to the same room instance should have very similar features. Therefore, we measure the Euclidian distance between the features of each pair of regions in order to form a similarity matrix $S\in \mathbb{R^{N\times N}}$ that indicates whether any given pair of regions belong to the same room instance. Element $S_{ij}$ classifies whether the region $f_i$ and $f_j$ belongs to the same room instance. After training, a statistical threshold is used to determine the room instance for inference.

Besides, the network output another semantic segmentation branch to classify every region into a room category. The most voted category in a room instance is determined as the room type.

Since the input features among multiple regions are less distinguishable even though we introduce the new Density Map features, the experiment shows that the deterministic network can hardly build an adequate criterion to split adjacent regions into different rooms. Therefore, we consider utilizing another generated adversarial network to introduce more distinguishable features to assist the original data. The wall information is a powerful feature for room instances and can be expressed simply by a binary mask. We build a pixel2pixel network reference in [---reference---] to generate the wall mask. Note that although the generated masks are usually not completed, full of burrs, and redundant, as shown in Figure [--- Figure--], our instance segmentation network can overcome the noises in the training process, which can hardly be accomplished by post-processing.

\section{Experiments}
  For demonstrating the efficacy and efficiency of our Uniform Regions, we conduct three floorplan based applications: 1) interior space planning which is a segmentation task, 2) structural similarity, and 3) floorplan generation. 

  \subsection{Interior Space Planning}
  The interior space planning task is important part of interior design and is used to determine how a space should be laid out and used. As shown in Figure[---figure--], a room in modern residential houses usually play multiple roles in human activities, such as meeting, media, dinning, entrance or balcony. These activities are seperately located in a room by considering some designing rules, e.g, the space size(meeting stands against long walls), position relation with other spaces(entrance neigbors with entry door, dining neigbors with kitchen, meeting is oposite to media), floorplan geometric shapes and the location of windows or doors. In limit space of residential house, the space planning usually has been considered for business floorplan designing, as a result, the interior space planning has nearly a deterministic solution in such a situation. This task can be viewed as a pre-task for interior scene synthesis task under complicated and practical residential floorplan. 

  \begin{table*}[tp]
    \fontsize{6.5}{8}\selectfont  
    \centering  
   \caption{Interior space planning experiment results on 3D-FRONT dataset. We report IoU \& F boundary score with and without outline metrics in the table. 1) The first row lists results using state-of-the-art methods under pixel level representation. 2) The second row lists results using different Encoder-Decoders under $(4\times 4\times0.5m)$ sub-Unit Region representation. 3) The third row lists results under different sub-Unit Region splitting strategies with Deeplab v3+ Encoder Decoder.}
   \label{tab:space_planning_main}
   \begin{tabular}{l|cccccc|cc}
 
     \toprule
     \multirow{3}*{Network} &
     \multicolumn{6}{c|}{IoU$\uparrow$} & \multicolumn{2}{c}{boundary F score$\uparrow$} \\
     \cline{2-9}
      {} & Mean &Living&Dining& Hallway & Entrance & Others& w/. outline& w/o. outline \\
     \midrule
     Deeplab v3+[] & 70.06& 88.04& 77.66& 71.02& 58.24& 55.32& 60.58& 23.69 \\
     HR-Net[] & 69.29& 88.12& 77.82& 69.36& 57.96& 53.2& 60.69& 22.42 \\
     UNet[] & 68.04& 85.62& 73.52& 68.66& 60.8& 51.6& 59.06& 23.58 \\
     DefGrid[] &- &- &- & -&- &- &- &- \\
     \midrule
     URE-Net(8)+Deeplab v3+ &72.32& 89.94& 80.02& 73.64& 60.74& 57.24& 72.71& 63.19 \\
     URE-Net(8)+HR-Net & 70.77& 89.5& 79.18& 72.92& 56.98& 55.28& 70.98& 61.85 \\
     URE-Net(8)+UNet & 70.5& 87.42& 76.46& 72.96& 62.08& 53.58& 71.26& 61.67 \\
     \midrule
     URE-Net(1)& 70.8& \textbf{90.26}& 74.42& \textbf{75.48}& 58.26& 55.58& 73.35& \textbf{68.17} \\
     URE-Net(2) & 71.9& 88.2& 78.6& 73.68& 62.1& 56.92& \textbf{73.62}& 66.34 \\
     URE-Net(4) & 72.05& 89.5& 79.12& 74.06& 61.74& 55.82& 72.85& 64.06 \\
     URE-Net(8) & \textbf{72.32}& 89.94& \textbf{80.02}& 73.64& 60.74& \textbf{57.24}& 72.71& 63.19 \\
     URE-Net(4.5) & 72.03& 89.12& 78.4& 74.12& \textbf{62.58}& 55.94& 71.03& 61.27 \\
     URE-Net(8.5) & 71.9& 89.72& 79.72& 73.24& 62.04& 54.76& 70.11& 58.98 \\

     \bottomrule
   \end{tabular}
 \end{table*}


\begin{table}[tp]
  \fontsize{6.5}{8}\selectfont  
  \centering  
 \caption{Ablation results on density map. We report the results with and without density map feature under pixel level(Deeplab v3+) and region level representation(URE-Net(8))}
 \label{tab:space_planning_ablation}
 \begin{tabular}{lc|c|cc}

   \toprule
   \multirow{3}*{Network} & \multirow{3}*{Density} &
   \multirow{3}*{mIoU$(\uparrow)$} & \multicolumn{2}{c}{boundary F score$(\uparrow)$} \\
   \cline{4-5}
    {} & {}& {} &w/ outline& w/o. outline \\
   \midrule
   Deeplab v3+ & - &69.54 &59.77& 19.63 \\
   Deeplab v3+ & \checkmark &\textbf{70.06} &\textbf{60.58}& \textbf{23.69}  \\
   \midrule
   URE-Net(8) &  - &71.60 &71.97& 62.72  \\
   URE-Net(8) & \checkmark &\textbf{72.32} &\textbf{72.71}& \textbf{63.19} \\

   \bottomrule
 \end{tabular}
\end{table}

  \textbf{Datasets.} Since the absent of dataset on the interior space planning tasks, we annotated the data based on 3D-FRONT dataset[--refrence--] which contains a collection of 6813 houses, populated with 3D furniture objects from the 3D-FUTURE dataset [--reference--]. The annotation is performed by professional designers and the original furnitures layout are refered. In our evaluation, we focus on the two room types: (i) living rooms, and (ii) dining rooms since the richness of space categories and complicated floorplan shapes. We filted out uncommon room floorplans or strange furnitures layout houses, and obtained 5340 rooms. The space planning dataset consists 9 categories of spaces, and the types and numbers of each category is shown in figure[---figure--]. 
  
  We merge several categories with too few numbers and use five categories in our experiments, including: (i) living, (ii) dining, (iii) entrance, (iv) hallway, and (v) others. We split 4272 and 1068 data for traning and testing respectively. We concatenate the raster room floorplan mask, door types mask and windows mask as inputs with $256 \times 256$ resolution and augment data on-the-fly by randomly flipping and rotating the images in interger times of 90 degrees.

  \textbf{Metrics.} The standard metric for semantic segmentatin is Intersection over Union(IoU), we calculate IoUs for each category and the Mean IoU(MIoU) for overall performance evaluation. Besides, the segmentation labels are generally a polygon shape and required to be vector format. The vectorization of segmentation result using previous segmentation methods suffers when the segmentation maps contain imperfections such as smoothed out corners and blury edges. The boundary regularity is important for the flollowing usage by designers or programs, since blury edges and fragmentation of regions are unacceptable. We thus also compute the Boundary F scores[---reference--] which calculates precision/recall between the predicted and ground-truth boundary, by allowing some distance threshold. And the average boundary F scores are calculated for overall categories. We reports results with threshold within 1 pixel with and without filtering the boundaries that coincides with room outline, since the outline is in fact the floorplan itself and can be easily derived from the input.
  
  \textbf{Comparison and Disccusion.} We did comparisons with state-of-the-art semantic segmentation networks: Deeplab v3+[--reference--], HR-Net[--reference--], and U-Net[--reference--], under the same backbone settings. We also compared with two recent works that focus on polygon or regular segmentation results: DefGrid[--reference--] and Curve-GCN[--reference--]. For the Uniform Regions network, we use Adam optimizer with a momentum of 0.9, a weight decay of 0.0005 and batch size 100. The learning rate is set 5e-4 and decays 0.1 every 30 epochs and. The optimization stops at 100 epochs. We use sub-Uniform Regions split under (4x4, 0.5) strategy. For the other networks, we follow the settings in original open-source code under pixel level segmentation. 

  Performances (IoUs and boundary F scores) are reported in Table \ref{tab:space_planning_main}. Our Unit Regions representation with any Encoder-Decoder(the second row) has a significant advantage over all the state-of-the-art networks(the first row). In terms of IoUs, the much better performence due to the smaller solution space. The advantage is much more obvious on the boundary F score without counting the floorplan outline, which indicates the shape of our results are more regular and similar to ground truth. This benefit from the geometric representation and region-aligned property. 

  From the second row of Table \ref{tab:space_planning_main}, we find URE-Net with Deeplab v3+ Encoder-Decoder has better performance. In following experiments we consistently adopt Deeplab v3+ as our Encoder-Decoder structure.

  To expolred the influence when using different splitting strategies of sub-Unit Regions, we train networks under six sppliting strategies: the spliting nums and minimal region threshs are (1x1, 1.0m), (2x2, 1.0m), (4x4, 1.0m), (4x4, 0.5m), (8x8, 1.0m), (8x8, 0.5m). The visualization of examples for each strategy are shown in Figure[--Figure--]. We use the Deeplab v3+ as our Encoder-Decoder for this comparison experiment and denote them as \textbf{URE-Net(1), URE-Net(2), URE-Net(4), URE-Net(4.5), URE-Net(8), URE-Net(8.5)}, respectively. In the third row of Table \ref{tab:space_planning_main}, We observe that the mean IoU performence of our network increases gradually with the sub-Unit Regions before URE-Net(8), and then decreases. The reason is that when using too few regions, space with difference features are forcedly limited in same region and the learning process would be confused. As the sub-region resolution increases, the representation ability would be released, meanwhile the solution space is also increased. As a result, the peroformance would slightly decreased. However we argue that the performence are consistently outperforms state-of-the-art under all sub-region resolution.

  We demonstrate the space planning visualization for each method in Figure[-figure-], our method is able to output much more regular results with less blury edges and rational planning.

  \textbf{Ablations.}
  The density map is a densely expressed and globally awared geometric information and can be easily concatenated with other inputs for traning. We explored the effect of density map both on pixel and region level representation. As shown in Table \ref{tab:space_planning_ablation}, the density map brings 0.52 and 0.72 mIoU increasing for pixel and region level representation. A more significant incresing to pixel level representation on boundary F score without outline can be observed, due to the regularity of the density map.


\subsection{Floorplan Retrieval}
  The floorplans are widely used for interior or architecture designs, to manage and analyze them, a floorplan retrieval method is essential. We test our method on the large-scale dataset RPLAN[--reference--] and compare with the state-of-the-art methods.

  \begin{table}[tp]
    \fontsize{6.5}{8}\selectfont  
    \centering  
   \caption{Floorplan retrieval results. The upper four results are reported in LayoutGMN[--ref--].}
   \label{tab:floorplan_retrieval}
   \begin{tabular}{l|c|c}
  
     \toprule
     \multirow{3}*{Method} & 
      \multicolumn{2}{c}{Method Test Accuracy on Triplets} \\
     \cline{2-3}
      {} &IoU-based$(\uparrow)$& User-based$(\uparrow)$ \\
     \midrule
     Graph Kernel & 92.07 &95.60  \\
     U-Net Triplet  & 93.01 &91.00   \\
     GCN-CNN Triplet  & 92.50 &91.80   \\
     LayoutGMN & 97.54 &97.60  \\
     \midrule
      URE-Net w/ density & 99.48 &98.62\\
      URE-Net w/o density & 99.3 &98.5\\
     \bottomrule
   \end{tabular}
  \end{table}

  \textbf{Datasets.}
  We use the RPLAN dataset for the floorplan retrieval task. The original dataset consists 80K floorplans and each floorplan is composed with multiple rooms and exterior and interior walls. The retrieval label that measures the similarity between different floorplans are approximated by IoU values of two layouts in LayoutGMN[--ref--]. Given an anchor layout, the threshold on IoU values to classify another layout as positive is 0.6. Negative examples are those that have a threshold value of at least 0.1 less than the positive ones. They filted out 7700 and 1588 data for traning and testing. They also annotated 452 triplets which better matches human's notion of structural similarity. We use both the IoU-based and user-based test dataset for evaluation.

  For data processing, we pack the room type, door mask, and density map that is calculated in each room seperately into multi-channel image with $256 \times 256$ resolution. Compared with space planning task, each room is viewed as a unit region in this experiment. Since each floorplan in this task consists not only the outline, the room layout are also important part for describing the floorplan, which are naturally isolated regions. 

  \textbf{Metrics.} The key to retrieval task is to generate an embedding feature for each floorplan, and the feature is exploited to measure as similarity with specified distance function, such as Euclidian or Cosine distance. Following the training process that classifies negative and positive floorplans towards certain anchor flooplan, we measure the classification accuracy based on Euclidian distance. 

\textbf{Comparison and Disccusion.}
We compare our method with four baselines:
\begin{itemize}
  \item \textbf{Graph Kernal(GK)[--ref--].} GK represents a 3D indoor scene into graph structures and compares substructures in the graph to capture similarity between the corresponding scenes. We adopt it to 2D layouts of floorplans.
  \item \textbf{U-Net[-ref--].} As one of the best segmentation networks, we use U-Net in a triplet network setting to auto-encode layout images. The input to the network is a multi-channel image with semantic segmentations
  \item \textbf{GCN-CNN[-ref-].} The state-of-the-art network for structural similarity on UI layouts is a hybrid network comprised of an attention-based GCN, similar to the gating mechanism in [28], coupled with a CNN.
  \item \textbf{LayoutGMN[-ref-].} LayoutGMN take each room and room connections as nodes and edges on a graph. They propose a graph matching network to evaluate the similarity between floorplans.
\end{itemize}
Results of the baslines are reported in LayoutGMN, and We train our method under the same data preparation. We use URE-Net with deeplab v3+ as our method. We use Adam optimizer with a momentum of 0.9, a weight decay of 0.0005 and batch size 10. The learning rate is set 1e-4 and decays 0.8 every 20 epochs and. The optimization stops at 200 epochs.

The experiments results are demonstrated in Table \ref{tab:floorplan_retrieval}, where our results outperforms all the other state-of-the-art methods. The aforementioned methods are based on either graph structures or semantic images. While graph structure requires hand-craft geometric features for each room node and edges(connections between rooms), and semantic images lack room relation and precise geometric information. Our method in fact plays a \emph{graph on image} function where we naturally represent each room as an unit region(graph node), meanwhile the features of each node are pooled from corresponding region on the semantic image. The geometric information of every room and the connection among rooms are completely encoded into node features. The symmetric function finally filts out the global representative and distinguishable features. We can also observe that the density map leads improvements in this task due to the dense geometric information.

\textbf{Visualization?}


\subsection{Floorplan Generation}
Floorplan generation generates rooms segmentation results for a given exterior wall boundary and front door. As introduced in aforementioned section \ref{tasks}, we format the floorplan generation as one-stage room instance segmentation. Besided, we employ another generated adversarial network to assist with distinguishable wall masks as extra input features. We show the generation results under our novel representation.

\textbf{Datasets.} We conduct the experiment on the commonly used RPLAN dataset. The input data for wall generation network is the exterior boundary, front door and the density map, while the output data is the interior walls mask. Then we pack the aforementioned input and output into multi-channel images and train the one-stage room segmentations. The segmentation is supervised by a room type classification and Euclidian distance with same room ids. 

The original datasets contains 13 kinds of rooms and we merge into 5 including Living, since the similar room characteristic(e.g., MasterRoom vs. SecondRoom) and too few proportions. Each room is split into sub-unit regions under $(8\times 8, 1m)$ strategy according Table \ref{tab:sub_region_split}, since it has better trade-off between IoU and region numbers. Each region is assinged with two labels: room type and room id, according to the the pixel labels in the region. We omit the wall types since our method directly take the boundary of these clustered regions as walls which is naturally a vector format. So the regions assigned with wall type are instead as the second statictic pixel label in the region. For those regions totally within certain walls, we select label the same as the closest region that has valid labels. We split the data into 75K and 5K for training and evaluation.

\textbf{Metrics.} Since the floorplan generation task is a highly non-trival problem, it's hard to evaluate the results objectively. Following method in Grpah2Plan(\hc{(refrence)}), we evaluate the quality of a sample of floorplans generated by our method in a user study. We asked users to select more plausible result in the mixed ground-truth floorplan and our results with the sampe boundary. 20 pairs of floorplans are randomly sampled from the test dataset and users could select either as more plausible or "Cannot tell". We asked 10 users to do the user study and the participants are professional designers for interior decoration. Besides, we demonstrate some visualization examples against the ground-truth in Figure()\hc{reference}).

\textbf{Comparison and Disccusion.}
Our training process is divided into three steps. In the first step, we use pix2pix to train a wall mask generation network on the training datasets for 100 epochs.
For the next step, we use URE-Net with deeplab v3+ to train room instance segmentation by using GT wall masks and other rasterized floorplan information as input for 100 epochs. 
In the above two steps, the learning rate is 0.0002 and decays 0.8 every 20 epochs.
Finally, we fine-tune the second step network to help the network reduce the domain gap between the generative wall masks and the GT wall masks. During fine-tuning, we randomly replace half of the input training GT wall masks with the generated wall masks. The initial learning rate of fine-tuning is 0.0001 and linearly decay to zero over 50 epochs. For each above steps, we use Adam optimizer with momentum of 0.9 and batch size 64.

We coolected 200 answers from 10 participants for the generated floorplan evaluation.The votes for different choices are: GT-(\hc{num}, ours-(\hc{num})) and cannot tell-(\hc{num}). This indicates that (\hc{num})\% participants think our results are more or equal plausible than the ground-truth. Figure (\hc{reference}) demonstrates examples of our results and GT, (\hc{waiting for the results})
